Dr.Quad at MEDIQA 2019: Towards Textual Inference and Question Entailment using contextualized representations

This paper presents the submissions by Team Dr.Quad to the ACL-BioNLP 2019 shared task on Textual Inference and Question Entailment in the Medical Domain. Our system is based on the prior work Liu et al. (2019) which uses a multi-task objective function for textual entailment. In this work, we explore different strategies for generalizing state-of-the-art language understanding models to the specialized medical domain. Our results on the shared task demonstrate that incorporating domain knowledge through data augmentation is a powerful strategy for addressing challenges posed by specialized domains such as medicine.

==> Models.tex <==
\section{Models}
In this section, we first provide a brief description about all the different models we used in the course of this work, followed by our approach in \S \ref{appraoch}.
\subsection{CBOW}
A continuous-bag-of-words model is used to encode the sentence into a single representation by simply averaging the word embeddings present in the sentence. This representation is then fed into an MLP to perform any type of classification on the sentence.
\subsection{Infersent}
\label{infersent}
\citet{conneau2017supervised} proposed Infersent which gets the sentence representations for both the premise \emph{U} and the hypothesis \emph{V} by running a bidirectional LSTM. Both these representations are passed to a fully connected layer by concatenating [U,V,|U-V|, U * V]. This model does well on many NLP tasks including NLI and thus offers a good starting point.

\subsection{BERT}
We also wanted to try deep contextualized word embeddings to verify if the robustness of the state of the art helps even without domain specific knowledge. We tried BERT\cite{devlin2018bert} as our contextualised embedding model. BERT is a transformer model which uses self attention. It has been found to capture good sentence representations, enabling it to get good accuracy. We tried this model and found some interesting results. We use the implementation of BERT found here\footnote{https://github.com/huggingface/pytorch-pretrained-BERT}
% \begin{figure}[ht]
% \centering
% \begin{minipage}{0.5\textwidth}
%   \centering
%   \includegraphics[width=\textwidth]{Bert.png}
%   \caption{BERT}
%   \label{fig:ernie}
% \end{minipage}%
% \end{figure}

\subsection{MT-DNN}
Deep contextualised word embeddings have become the norm to get state of the art performance. \cite{liu2019multi} proposed a multi task set up of BERT to get state of the art results on SNLI\cite{bowman2015large} and MNLI\cite{williams2017broad}. The authors have proved empirically that the model is very good at domain adaptation and is able to get very good results with very small training data because of its ability to generalise. We use the MT-DNN implementation open-sourced\footnote{https://github.com/namisan/mt-dnn} by the authors.



==> RealtedWork.tex <==
\section{Related Work}

In this section, we briefly discuss the prior work in each of our subtasks.
\paragraph{NLI:}  Natural language inference is a widely studied problem. With the introduction of benchmark datasets such as SNLI \cite{bowman2015large} and Multi-NLI \cite{williams2017broad}, the community has seen diverse approaches. Prior work ranges from traditional methods such as CBOW and simple BiLSTM baselines \cite{nangia2017repeval} to the more recent deep neural network methods such as ESIM \cite{chen2016enhanced}, Infersent \cite{conneau2017supervised}. To test the generalizability of state-of-the-art NLI models across diverse domains, \citet{romanov2018lessons} introduce a new dataset MedNLI for clinical domain.They explore transfer learning techniques from other NLI datasets such as SNLI, Multi-NLI in order to learn more about the entailment task itself.

\paragraph{RQE:} Recognising textual entailment has been widely addressed in the past\cite{dagan2013recognizing}. FAQ Finder\cite{burke1997question} was one of the very first systems to use question entailment to answer related questions. Traditional feature based engineering has been extensively used in the form of using syntax parsing\cite{wang2009syntactic} for finding similar questions. \citet{shah2018adversarial} take an adversarial approach for a similar task of identifying duplicate questions. More recent work has focused on using neural models for identifying duplicated/related questions.\cite{devlin2018bert,liu2019multi}


 \paragraph{QA:} 
 %With the advent of large Question-Answering (QA) datasets research in this area has seen a surge of interest in the past few years, across various domains. Common examples include Wikipedia articles \cite{squad,wikireading,wikisuggest}, news articles \cite{newsqa, attentive}  trivia questions \cite{triviaqa}, exam questions \cite{race}, and stories \cite{cbtgoldilocks}. In the medical domain, datasets such as MEDQUAD \cite{019arXiv190108079A} and CliCR \cite{vsuster2018clicr} have recently been introduced. These reading comprehention challenges differ on various aspects such as answer types, passage lengths. In this work, we focus on the CliCR challenge which belongs to the cloze-style reading comprehention category. It is similar to the setup of CNN/DailyMail \cite{cbtgoldilocks, attentive} where the answers are a set of entities and the task is to fill the blank in the question. 

Question Re-ranking has been addressed in the form of syntactic alignment of the passage with the question\cite{aktolga2011passage}. Question type identification has also been used while re-ranking\cite{aktolga2011passage}. \citet{chen2006reranking} have tried to use language modelling to pick the results of re-rank the answers. 

    % \item Add related work on NLI models. One paragraph about NLI in Medical domain.
    % \item Add related work on question entailment/ duplicate identification, including for medical domain.
    % \item Add related work for methods of question re-ranking.
    


==> Results.tex <==
\section{Results}
  

% \subsection{NLI}
% \begin{enumerate}
% \item Features include with baseline models
%     \begin{itemize}
%         \item Abbreviation: As discussed before the motivation of expanding abbreviations was to allow greater lexical overlap between the premise and hypothesis. A simple error analysis showed most of the baseline and robust models missed out on entailments when either of premise or hypothesis used abbreviated terms.
%         \item Metamap: \textcolor{blue}{TODO - Metamap explanation}
%     \end{itemize}
% % \item Bert
% % \item MT-DNN
% \end{enumerate}

% \begin{table}[h]
% \small
% \begin{center}
% \begin{tabular}{|l|l|l|l|l|}
% \hline \bf  & \bf Train & \bf Dev & \bf Test & \bf Total\\ \hline
%  Matches  & 99 & 9 & 115 & 233\\

% \hline
% \end{tabular}
% \end{center}
% \caption{\label{} Matches found in sets for abbreviation}
% \end{table}



\subsubsection{Re-Ranking}
\begin{enumerate}
    \item BM25 baseline
    \item Leverage RQE + NLI from re-rank
    \item CliCR trained re-ranker for this task
\end{enumerate}
\subsection{CliCR}
\begin{enumerate}
    \item Use NLI model for CLiCR
\end{enumerate}

==> researchQ.tex <==
\section{Research Questions}
\label{resQ}

In our work, we plan to answer the following research questions:
\begin{enumerate}
    \item \textbf{Can textual entailment (TE)  or natural language inference (NLI) help QA systems?} \\
    TE or NLI is the task of understanding the relation between two text fragments, whether two text fragments (sentences) \textit{entail}, \textit{contradict} each other or none of the above. Prior work \cite{dagan2006pascal, demszky2018transforming} has shown close relations between the NLI and QA tasks. \citet{demszky2018transforming} transform existing QA datasets to augment and diversify NLI datasets. Inspired by their findings, we plan to transform questions-answers from the QA dataset into premise-hypothesis pairs and use existing NLI models for answering a questions. We hypothesize that such an approach would allow for model interpretability. For instance, the sentences from the context document to which the answer entails the best, will form as the supporting evidence.  We hypothesize that such an approach will provide the transparency which is much required in QA systems. Additionally, we also plan to explore the use of NLI as a re-ranker on top of existing QA systems.
    \item \textbf{How to incorporate domain knowledge in generic systems?}\\
   With the advent of deep neural models such as BERT \cite{devlin2018bert}, MT-DNN \cite{liu2019multi}, it is but natural to use these off-the-shelf models for the task at hand. However, these models have been pre-trained on a few domains. The challenge still remains on how these models generalize to new domains. Medical domain is especially challenging, for instance  \citet{romanov2018lessons} show how word embeddings trained on Common Crawl are ineffective for this domain. \citet{abacha2016recognizing} experiment with different domain features such as medical named entity recognition,  UMLS \cite{bodenreider2004unified} with a feature-based machine learning model. In this work, we explore how to marry such domain features with state-of-the-art models. 
\end{enumerate}
